Bandwidth Extension on Raw Audio via Generative Adversarial Networks

Neural network-based methods have recently demonstrated state-of-the-art results on image synthesis and super-resolution tasks, in particular by using variants of generative adversarial networks (GANs) with supervised feature losses. Nevertheless, previous feature loss formulations rely on the availability of large auxiliary classifier networks, and labeled datasets that enable such classifiers to be trained. Furthermore, there has been comparatively little work to explore the applicability of GAN-based methods to domains other than images and video. In this work we explore a GAN-based method for audio processing, and develop a convolutional neural network architecture to perform audio super-resolution. In addition to several new architectural building blocks for audio processing, a key component of our approach is the use of an autoencoder-based loss that enables training in the GAN framework, with feature losses derived from unlabeled data. We explore the impact of our architectural choices, and demonstrate significant improvements over previous works in terms of both objective and perceptual quality.

==> background.tex <==

\section{Background}
\label{sec:background}

\paragraph{Audio Bandwidth Extension.}
Audio super-resolution is the task of constructing a high-resolution audio signal from a low-resolution signal that contains a fraction of the original samples.
Concretely, given a low-resolution sequence of audio samples $x_{l}~=~(x_{1/R_{l}}, \ldots, x_{R_{l}T/R_{l}})$, we wish to synthesize a high-resolution audio signal $x_{h}~=~(x_{1/R_{h}}, \ldots, x_{R_{h}T/R_{h}})$, where $R_{l}$ and $R_{h}$ are the sampling rates of the low and high-resolution signals, respectively.
We denote $r = R_h/R_l$ as the \textit{upsampling ratio}, which ranges from 2 to 6 in this work.
Note that since the bandwidth of a signal sampled at rate $R$ is limited to the Nyquist frequency $R/2$, audio super-resolution is equivalent to reconstructing the missing frequency content between frequencies $R_l/2$ and $R_h/2$.

\paragraph{GANs for Super-Resolution}
GANs developed for super-resolution tasks have several important differences compared to the original formulation of \cite{goodfellow_nips14}.
When used to generate new instances from a modeled data distribution $\pdata$, the generator ($G$) parameterized by $\theta_G$ learns the mapping to data space as $G(\bm{z}; \theta_G)$, where $\bm{z}$ is a low-dimensional latent vector sampled from a noise prior.
The discriminator ($D$) parameterized by $\theta_D$ then estimates the probability that $G(\bm{z}; \theta_G)$ was drawn from $\pdata$ rather than the generator distribution $p_g$.
In contrast, for deterministic super-resolution, $G$ is no longer conditioned on noise and learns the mapping to high-resolution data space $p_h$ as $G(\bm{x_l}; \theta_G)$, where $\bm{x_l}$ is drawn from the low-resolution data distribution $p_l$.
The task of $D$ is to discriminate between samples drawn from the high-resolution and super-resolution (generator) distributions $p_h$ and $p_g$, respectively.
Since low-resolution data $\bm{x_l}$ corresponds directly to downsampled, high-resolution data $\bm{x_h}$ during training, we expect $G(\bm{x_l}; \theta_G) \approx \bm{x_h}$.
This is in contrast to general GANs where $G(\bm{z}; \theta_G)$ is ideally dissimilar to instances from the training set.
$G$ and $D$ are optimized according to the two-player minimax problem:

\begin{equation}
\label{eq:minimax}
\underset{\theta_G}{\text{min}}~\underset{\theta_D}{\text{max}}~
\E_{\bm{x_h} \sim p_h(\bm{x_h})} \left[ \log D\left(\bm{x_h}; \theta_D \right)\right] +
\E_{\bm{x_l} \sim p_l(\bm{x_l})} \left[ \log (1 - D\left(G\left(\bm{x_l}; \theta_G \right)\right) ) \right]
\end{equation}

This framework enables a joint optimization of two neural networks - $G$ generates super-resolution data with the goal of fooling $D$, and $D$ is trained to distinguish between real and super-resolved data.
Thus, the GAN approach encourages $G$ to learn solutions that are hard to distinguish from real, high-resolution data.
Compared to networks trained with conventional losses that result in over-smoothed outputs (i.e., \textit{regression-to-the-mean}\tocite), GANs synthesize sharp, detailed outputs that lie along the manifold of natural data.

\paragraph{Feature Losses}

Recent work has shown that generation of perceptually relevant detail can be improved by augmenting or replacing conventional pixel-wise losses with metrics computed in the feature spaces of pre-trained auxiliary neural networks.
These \textit{feature losses} (also called perceptual losses) have been applied almost exclusively for images, for instance in variational generation and network inversion \cite{dosovitskiy_nips16}, super-resolution \cite{ledig_cvpr17}, and style transfer \cite{gatys_arxiv15, gatys_cvpr16}.
If we denote the tensor after convolutional layer $j$ of the auxiliary network as $\phi_j(.)$, then a generic feature loss has the form:

\begin{equation}
\label{eq:feat_loss}
\mathcal{L}_{feat,j} = \sum_{x=1}^{N_j} \sum_{y=1}^{M_j} \sum_{z=1}^{C_j} \left( \phi_j(\bm{y})_{x,y,z} - \phi_j(\bm{\hat y})_{x,y,z} \right)^2,
\end{equation}

where $N_j$, and $M_j$, and $C_j$ denote the dimensions of the output feature tensor for layer $j$, and $\bm{y}$ and $\bm{\hat y}$ are the groundtruth and estimated data, respectively.

Our approach also uses a feature loss to induce perceptually-relevant texture details, however our method is the first to explore non-classifier-based feature losses.

